Fast and Simple Computation of All Longest Common Subsequences

This paper shows that a simple algorithm produces the {\em all-prefixes-LCSs-graph} in $O(mn)$ time for two input sequences of size $m$ and $n$. Given any prefix $p$ of the first input sequence and any prefix $q$ of the second input sequence, all longest common subsequences (LCSs) of $p$ and $q$ can be generated in time proportional to the output size, once the all-prefixes-LCSs-graph has been constructed. The problem can be solved in the context of generating all the distinct character strings that represent an LCS or in the context of generating all ways of embedding an LCS in the two input strings.

==> bilabial-anticanon-tab.tex <==
{\setlength{\unitlength}{.02em}\thicklines
\begin{picture}(950,850)(-25,-825)
\drawline(100,-775)(100,-725)
\drawline(100,-675)(100,-625)
\drawline(100,-575)(100,-525)
\drawline(100,-475)(100,-425)
\drawline(100,-375)(100,-325)
\drawline(100,-275)(100,-225)
\drawline(100,-175)(100,-125)
\drawline(125,-100)(175,-100)
\drawline(225,-100)(275,-100)
\drawline(325,-100)(375,-100)
\drawline(425,-100)(475,-100)
\drawline(525,-100)(575,-100)
\drawline(625,-100)(675,-100)
\drawline(725,-100)(775,-100)
\drawline(825,-100)(875,-100)
\drawline(200,-775)(200,-725)
\drawline(200,-675)(200,-625)
\drawline(200,-575)(200,-525)
\drawline(200,-475)(200,-425)
\drawline(225,-400)(275,-400)
\drawline(300,-375)(300,-325)
\drawline(325,-300)(375,-300)
\drawline(425,-300)(475,-300)
\drawline(525,-300)(575,-300)
\drawline(625,-300)(675,-300)
\drawline(725,-300)(775,-300)
\drawline(825,-300)(875,-300)
\drawline(325,-800)(375,-800)
\drawline(400,-775)(400,-725)
\drawline(400,-675)(400,-625)
\drawline(400,-575)(400,-525)
\drawline(400,-475)(400,-425)
\drawline(425,-400)(475,-400)
\drawline(525,-400)(575,-400)
\drawline(625,-400)(675,-400)
\drawline(725,-400)(775,-400)
\drawline(825,-400)(875,-400)
\drawline(625,-800)(675,-800)
\drawline(700,-775)(700,-725)
\drawline(725,-700)(775,-700)
\drawline(825,-700)(875,-700)
\put(100,0){\makebox(0,0){\shortstack{1\\{\strut\bf b}}}}
\put(200,0){\makebox(0,0){\shortstack{2\\{\strut\bf a}}}}
\put(300,0){\makebox(0,0){\shortstack{3\\{\strut\bf l}}}}
\put(400,0){\makebox(0,0){\shortstack{4\\{\strut\bf a}}}}
\put(500,0){\makebox(0,0){\shortstack{5\\{\strut\bf c}}}}
\put(600,0){\makebox(0,0){\shortstack{6\\{\strut\bf l}}}}
\put(700,0){\makebox(0,0){\shortstack{7\\{\strut\bf a}}}}
\put(800,0){\makebox(0,0){\shortstack{8\\{\strut\bf v}}}}
\put(900,0){\makebox(0,0){\shortstack{9\\{\strut\bf a}}}}
\put(0,-100){\makebox(0,0){1 {\bf b}}}
\thicklines\put(100,-100){\circle{50}}
\put(100,-100){\makebox(0,0){1}}
\put(200,-100){\makebox(0,0){1}}
\put(300,-100){\makebox(0,0){1}}
\put(400,-100){\makebox(0,0){1}}
\put(500,-100){\makebox(0,0){1}}
\put(600,-100){\makebox(0,0){1}}
\put(700,-100){\makebox(0,0){1}}
\put(800,-100){\makebox(0,0){1}}
\put(900,-100){\makebox(0,0){1}}
\put(0,-200){\makebox(0,0){2 {\bf i}}}
\put(100,-200){\makebox(0,0){1}}
\put(200,-200){\makebox(0,0){1}}
\put(300,-200){\makebox(0,0){1}}
\put(400,-200){\makebox(0,0){1}}
\put(500,-200){\makebox(0,0){1}}
\put(600,-200){\makebox(0,0){1}}
\put(700,-200){\makebox(0,0){1}}
\put(800,-200){\makebox(0,0){1}}
\put(900,-200){\makebox(0,0){1}}
\put(0,-300){\makebox(0,0){3 {\bf l}}}
\put(100,-300){\makebox(0,0){1}}
\put(200,-300){\makebox(0,0){1}}
\thicklines\put(300,-300){\circle{50}}
\put(300,-300){\makebox(0,0){2}}
\put(400,-300){\makebox(0,0){2}}
\put(500,-300){\makebox(0,0){2}}
\thinlines\put(600,-300){\circle{50}}
\put(600,-300){\makebox(0,0){\bf 2}}
\put(700,-300){\makebox(0,0){2}}
\put(800,-300){\makebox(0,0){2}}
\put(900,-300){\makebox(0,0){2}}
\put(0,-400){\makebox(0,0){4 {\bf a}}}
\put(100,-400){\makebox(0,0){1}}
\thicklines\put(200,-400){\circle{50}}
\put(200,-400){\makebox(0,0){2}}
\put(300,-400){\makebox(0,0){2}}
\thicklines\put(400,-400){\circle{50}}
\put(400,-400){\makebox(0,0){3}}
\put(500,-400){\makebox(0,0){3}}
\put(600,-400){\makebox(0,0){3}}
\thinlines\put(700,-400){\circle{50}}
\put(700,-400){\makebox(0,0){3}}
\put(800,-400){\makebox(0,0){3}}
\thinlines\put(900,-400){\circle{50}}
\put(900,-400){\makebox(0,0){\bf 3}}
\put(0,-500){\makebox(0,0){5 {\bf b}}}
\thinlines\put(100,-500){\circle{50}}
\put(100,-500){\makebox(0,0){\bf 1}}
\put(200,-500){\makebox(0,0){2}}
\put(300,-500){\makebox(0,0){2}}
\put(400,-500){\makebox(0,0){3}}
\put(500,-500){\makebox(0,0){3}}
\put(600,-500){\makebox(0,0){3}}
\put(700,-500){\makebox(0,0){3}}
\put(800,-500){\makebox(0,0){3}}
\put(900,-500){\makebox(0,0){3}}
\put(0,-600){\makebox(0,0){6 {\bf i}}}
\put(100,-600){\makebox(0,0){1}}
\put(200,-600){\makebox(0,0){2}}
\put(300,-600){\makebox(0,0){2}}
\put(400,-600){\makebox(0,0){3}}
\put(500,-600){\makebox(0,0){3}}
\put(600,-600){\makebox(0,0){3}}
\put(700,-600){\makebox(0,0){3}}
\put(800,-600){\makebox(0,0){3}}
\put(900,-600){\makebox(0,0){3}}
\put(0,-700){\makebox(0,0){7 {\bf a}}}
\put(100,-700){\makebox(0,0){1}}
\thinlines\put(200,-700){\circle{50}}
\put(200,-700){\makebox(0,0){\bf 2}}
\put(300,-700){\makebox(0,0){2}}
\thinlines\put(400,-700){\circle{50}}
\put(400,-700){\makebox(0,0){\bf 3}}
\put(500,-700){\makebox(0,0){3}}
\put(600,-700){\makebox(0,0){3}}
\thicklines\put(700,-700){\circle{50}}
\put(700,-700){\makebox(0,0){4}}
\put(800,-700){\makebox(0,0){4}}
\thinlines\put(900,-700){\circle{50}}
\put(900,-700){\makebox(0,0){\bf 4}}
\put(0,-800){\makebox(0,0){8 {\bf l}}}
\put(100,-800){\makebox(0,0){1}}
\put(200,-800){\makebox(0,0){2}}
\thicklines\put(300,-800){\circle{50}}
\put(300,-800){\makebox(0,0){\bf 3}}
\put(400,-800){\makebox(0,0){3}}
\put(500,-800){\makebox(0,0){3}}
\thicklines\put(600,-800){\circle{50}}
\put(600,-800){\makebox(0,0){\bf 4}}
\put(700,-800){\makebox(0,0){4}}
\put(800,-800){\makebox(0,0){4}}
\put(900,-800){\makebox(0,0){4}}
\end{picture}}


==> bilabial-anticanon-tte.tex <==
\\\mathtt{b^{1}_{1}a^{4}_{2}a^{7}_{4}l^{8}_{6}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{7}_{4}l^{8}_{6}}
\\\mathtt{b^{1}_{1}l^{3}_{6}a^{4}_{7}a^{7}_{9}}


==> bilabial-anticanon-ttl.tex <==
\\\mathtt{baal}
\\\mathtt{blal}
\\\mathtt{blaa}


==> bilabial-embeddings-tte.tex <==
\\\mathtt{b^{1}_{1}a^{4}_{2}a^{7}_{4}l^{8}_{6}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{7}_{4}l^{8}_{6}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{4}_{4}l^{8}_{6}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{4}_{4}a^{7}_{7}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{4}_{4}a^{7}_{9}}
\\\mathtt{b^{1}_{1}l^{3}_{3}a^{4}_{7}a^{7}_{9}}
\\\mathtt{b^{1}_{1}l^{3}_{6}a^{4}_{7}a^{7}_{9}}

